Learning to Reason With Relational Abstractions

Large language models have recently shown promising progress in mathematical reasoning when fine-tuned with human-generated sequences walking through a sequence of solution steps. However, the solution sequences are not formally structured and the resulting model-generated sequences may not reflect the kind of systematic reasoning we might expect an expert human to produce. In this paper, we study how to build stronger reasoning capability in language models using the idea of relational abstractions. We introduce new types of sequences that more explicitly provide an abstract characterization of the transitions through intermediate solution steps to the goal state. We find that models that are supplied with such sequences as prompts can solve tasks with a significantly higher accuracy, and models that are trained to produce such sequences solve problems better than those that are trained with previously used human-generated sequences and other baselines. Our work thus takes several steps toward elucidating and improving how language models perform on tasks requiring multi-step mathematical reasoning.

==> sections/datasets.tex <==
\section{Datasets}

\subsection{Task 1: Unit Conversion}

The unit conversion task involves converting a given quantity and unit, then finding the equivalent quantity in another unit based on the conversion rules that are provided in the prompt.
The conversion rules are presented in random order, and can collectively be viewed as edges of a graph.
Solving the task, then, is equivalent to finding a path from the source node to the destination node while performing the corresponding multiplication (forward) and division (backward) operations when traversing each edge.
The task is presented as a sequence completion task using the graph description and the conversion instructions as the prompt (see example in Table \ref{table:uc_dataset} under \textbf{Prompt}).
Depending on the experimental condition, the model would be trained to produce a target sequence which would describe the path traversed and the arithmetic operations involved.

We trained the model using 4 target sequence types based on the structure of each conversion (edge traversal) step:
\begin{enumerate}
    \item Units first: state the source and destination units of the traversing edge, followed by the numerical expression
    \item Numbers first: state the numerical expression, followed by the source and destination units
    \item Interleaved: state the source quantity and unit, then the remainder of the numerical expression, followed by the destination unit
    \item Numbers only: state the numerical expression only
\end{enumerate}

For each sequence type, we also compared whether having the model produce an abstract plan involving units only would be helpful.
Overall, we had 4 (step types) x 2 (plan vs no plan) = 8 conditions in comparison.

To maintain consistent difficulty across our analyses, we used graphs with 10 nodes and 12 edges, and problems that could be solved using exactly 5 edge traversals.
All arithmetic in this task was performed in modulo-5 to avoid the arbitrary fractions and large numbers that would result from compounding of multiplication and division operations involved in multi-step problems.
This allowed us to focus on the reasoning component of the task rather than the numerical accuracy of performing long arithmetic operations.

\input{tables/uc_dataset}

\subsection{Task 2: Grade School Math}
